Search for New Physics in Dijet Mass and Angular Distributions in pp Collisions at sqrt(s) = 7 TeV Measured with the ATLAS Detector

A search for new interactions and resonances produced in LHC proton-proton (pp) collisions at a centre-of-mass energy sqrt(s)= 7 TeV has been performed with the ATLAS detector. Using a data set with an integrated luminosity of 36 pb-1 dijet mass and angular distributions have been measured up to dijet masses of \sim 3.5 TeV and found to be in good agreement with Standard Model predictions. This analysis sets limits at 95% C.L. on various models for new physics: an excited quark is excluded with mass between 0.60 and 2.64 TeV, an axigluon hypothesis is excluded for axigluon masses between 0.60 and 2.10 TeV and Randall-Meade quantum black holes are excluded in models with six extra space-time dimensions for quantum gravity scales between 0.75 and 3.67 TeV. Production cross section limits as a function of dijet mass are set using a simplified Gaussian signal model to facilitate comparisons with other hypotheses. Analysis of the dijet angular distribution using a novel technique 18 simultaneously employing the dijet mass excludes quark contact interactions with a compositeness scale {\Lambda} below 9.5 TeV.

==> Makefile <==
LATEX    = latex
BIBTEX   = bibtex
DVIPS    = dvips

BASENAME = DiJetMassAngle

default: testpdflatex

testlatex:
	latex  ${BASENAME}
	latex  ${BASENAME}
	bibtex ${BASENAME}
	latex  ${BASENAME}
	latex  ${BASENAME}
	latex  ${BASENAME}
	dvipdf -sPAPERSIZE=a4 -dPDFSETTINGS=/prepress ${BASENAME}

#	dvips ${BASENAME}
#	ps2pdf ${BASENAME}.ps
#	mv ${BASENAME}.dvi output/
#	mv ${BASENAME}.pdf output/
#
#   Now do Appendices
#
#	latex Appendix_res
#	latex Appendix_ang
#	dvipdf Appendix_res
#	dvipdf Appendix_ang
	make clean

testpdflatex:
	pdflatex  ${BASENAME}
	pdflatex  ${BASENAME}
	bibtex    ${BASENAME}
	pdflatex  ${BASENAME}
	pdflatex  ${BASENAME}
	pdflatex  ${BASENAME}
#	mv ${BASENAME}.pdf output/
	make clean

#
# standard Latex targets
#

%.dvi:	%.tex 
	$(LATEX) $<

%.bbl:	%.tex *.bib
	$(LATEX) $*
	$(BIBTEX) $*

%.ps:	%.dvi
	$(DVIPS) $< -o $@

%.pdf:	%.tex
	$(PDFLATEX) $<

.PHONY: clean

clean:
	rm -f *.aux *.log *.blg *.brf *.cb *.ind *.idx *.ilg  \
	      *.inx *.dvi *.toc *.out *~ ~* spellTmp ${BASENAME}.ps figures/*.aux


